Well-calibrated Confidence Measures for Multi-label Text Classification with a Large Number of Labels

We extend our previous work on Inductive Conformal Prediction (ICP) for multi-label text classification and present a novel approach for addressing the computational inefficiency of the Label Powerset (LP) ICP, arrising when dealing with a high number of unique labels. We present experimental results using the original and the proposed efficient LP-ICP on two English and one Czech language data-sets. Specifically, we apply the LP-ICP on three deep Artificial Neural Network (ANN) classifiers of two types: one based on contextualised (bert) and two on non-contextualised (word2vec) word-embeddings. In the LP-ICP setting we assign nonconformity scores to label-sets from which the corresponding p-values and prediction-sets are determined. Our approach deals with the increased computational burden of LP by eliminating from consideration a significant number of label-sets that will surely have p-values below the specified significance level. This reduces dramatically the computational complexity of the approach while fully respecting the standard CP guarantees. Our experimental results show that the contextualised-based classifier surpasses the non-contextualised-based ones and obtains state-of-the-art performance for all data-sets examined. The good performance of the underlying classifiers is carried on to their ICP counterparts without any significant accuracy loss, but with the added benefits of ICP, i.e. the confidence information encapsulated in the prediction sets. We experimentally demonstrate that the resulting prediction sets can be tight enough to be practically useful even though the set of all possible label-sets contains more than $1e+16$ combinations. Additionally, the empirical error rates of the obtained prediction-sets confirm that our outputs are well-calibrated.

==> Sections/Section_pool.tex <==
\begin{abstract}
We extend our previous work on the application of Conformal Prediction (CP) to the task of multi-label text classification and present experimental results on two English and one Czech language data-sets. Specifically, we combine the Inductive Conformal Prediction (ICP) version of the framework with three deep neural network classifiers of two types: one based on contextualised (BERT) and two on non-contextualised word-embeddings. Following the label powerset ICP approach, we assign nonconformity scores to label-sets from which the corresponding p-values and prediction-sets are determined and we experiment with 3 different versions of $L_p$  nonconformity measure. Our experimental results show that the contextualised-based classifier surpasses the non-contextualised-based ones and that the performance of the underlying classifiers is carried out on their ICP counterparts without any significant accuracy loss. The added benefits of ICP is prediction-specific confidence information is given in Prediction-sets can be tight enough to be practically useful even though the set of possible label-sets contains tens of thousands of label combinations. Additionally, the empirical error rates of the obtained prediction-sets confirm that our outputs are well-calibrated. Moreover, we present a preliminary attempt at addressing the computational inefficiency problem arising from the need of evaluating the p-values of a~huge number of possible label-sets, by eliminating from consideration a significant number of label-sets that will surely have a p-value below the specified significance level.
\end{abstract}

% As harris made it
\subsection{CP in the Multi-label Setting}
\label{sec:cp_in_the_multi-label_setting}

%Harris: The label-set is an element of the powerset not a subset. The prediction sets we produce are subsets of the powerset!!
Unlike the multi-class classification setting, in multi-label classification each instance can belong to multiple classes, e.g. a news-wire might be tagged under both \emph{politics} and \emph{economy}. Therefore the true classification (\emph{label-set}) $y_{n+m}$ of each instance $x_{n+m}$ is a set $Y_i \in \mathcal{P}\{\Psi_1, \dots, \Psi_d\}$ \footnote{The powerset of a set A, i.e. $\mathcal{P}(A)$, is a set that contains all subsets of $A$ including $\emptyset.$ and $A$ itself.}, where $\Psi_1, \dots, \Psi_d$ are the unique classes.

Different variations of CP have been proposed for handling multi-label classification problems through problem reformulation. These include decomposing each multi-label instance into a number of single-label examples (\emph{Instance Reproduction} (IR)) \citep{wang:Instance_Reproduction2014}; or decomposing the problem into several independent binary classification problems - one for each unique class (\emph{Binary-Relevance} (BR)) \citep{wang:mlcp,lambr:brmlcp} or transforming the problem into a multi-class one by treating each label-set as a unique class (\emph{Label Powerset} (LP)) \citep{papa:mlcp}.

As the standard guarantee provided by CP is that $P(y_{n+m} \notin \Gamma^\epsilon_{x_{n+m}}) \leq \epsilon$ and since in the multi-label setting $y_{n+m}$ is a label-set, the natural extension of CP to multi-label classification is for the prediction set $\Gamma^\epsilon_{x_{n+m}}$ to correspond to a set of label-sets, i.e. $\Gamma^\epsilon_{x_{n+m}} \subseteq \mathcal{P}(\{Y_1, \dots, Y_d\})$, with at most $\epsilon$ chance of not containing the true label-set $y_{n+m}$. This is the guarantee provided by the approaches proposed in \citep{lambr:brmlcp} and \citep{papa:mlcp}. The other variations on the other hand provide somewhat weaker guarantees. Specifically, the approaches proposed in \citep{wang:Instance_Reproduction2014} and \citep{wang:mlcp} provide a prediction set $\Gamma^\epsilon_{x_{n+m}} \in \mathcal{P}(\{Y_1, \dots, Y_d\})$ with the guarantee that the chance of it not containing any element of $y_{n+m}$ is at most $\epsilon$, i.e. $ \forall Y_j \in y_{n+m} \implies P( Y_j \notin \Gamma^\epsilon_{x_{n+m}}) \leq \epsilon$. This does not include any bound on the chance of $\Gamma^\epsilon_{x_{n+m}}$ containing labels that are not in $y_{n+m}$.

% These implementations refer to two different versions of CP prediction-set output. IR \citep{wang:Instance_Reproduction2014}, and BR \citep{wang:mlcp}, \citep{lambr:brmlcp} as originally proposed, output a \emph{prediction region}, that is a single label-set $\Gamma^\epsilon_{x_{n+1}}$ that includes all classes $\Psi_j$ assigned to them p-values $p_{x_{n+1}}^{\Psi_j}$ that satisfy the predefined significance level $\epsilon$. The prediction region in the IR case is defined as  $\Gamma^\epsilon_{x_{n+1}} = \{ \Psi_j : p_{x_{n+1}}^{\Psi_j} > \epsilon, j = 1, \dots, d \}$ and in BR case as $\Gamma^\epsilon_{x_{n+1}} = \{ \Psi_j : p_{x_{n+1}}^{\Psi_j} > \frac{\epsilon}{d}, j = 1, \dots, d\}$, where $p_{x_{n+1}}^{\Psi_j}$ refers to the to the corresponding p-values of each implementation. The differentiation of prediction region definition in the BR implementation ($ \frac{\epsilon}{d} $ instead of $ \epsilon $) is derived from the Bonferroni general inequality that is used for the synthesis of multiple statistical conclusions - one for each class $\Psi_j$ in the BR case. The virtue of CP, also known as the calibration property of CP, is that all classes included in the true label-set are also included in the prediction region, bound by significance level $\epsilon$, i.e. : $ \forall \Psi_j \in y_{n+1} \implies P( \Psi_j \notin \Gamma^\epsilon_{x_{n+1}}) \leq \epsilon$. On the other hand, the output of the power-set implementation \citep{papa:mlcp}, is a \emph{set-prediction}, that is a set that includes all label-sets $Y_j \in \mathcal{P}(\{\Psi_1, \dots, \Psi_d\})$ assigned to them p-values $p_{x_{n+1}}^{Y_j}$ that satisfy the predefined significance level $\epsilon$, i.e. $\Gamma^\epsilon_{x_{n+1}} = \{Y_j : p_{x_{n+1}}^{Y_j} > \epsilon\}$. In such a setting the virtue of CP is  $ P(y_{n+1} \notin \Gamma^\epsilon_{x_{n+1}}) \leq \epsilon$. 

In this work we follow the LP approach proposed in \citep{papa:mlcp}. The reason for this choice is twofold. Firstly, we want our approach to provide equally strong guarantees as those provided by CP in other settings and secondly, the LP transformation has the added advantage of enabling the development of more accurate nonconformity measures by taking label correlations into account, as opposed to dealing with each class individually. The main disadvantage of LP is its computational complexity with respect to the number of unique classes, which grows exponentially. For this reason we follow the inductive version of the CP framework and propose a modification of the original approach that provides significant gains in terms of computational efficiency while producing exactly the same outputs.

%In this work we focused only on the set-prediction version of ICP as originally proposed by \cite{papa:icm-rr} (LP approach). In different case, modifications would be required to the well studied from bibliography for the task of multi-label text classification architecture of the utilised underlying models (bert, randinit and word2vec). Also, for the IR and BR implementations, cases which are frequently encountered in multi-label scenario, such as with class imbalance in the distribution of instances and with class dependence to each other may cause performance decrease to the final classification output. In addition for the BR implementation, when dealing with problems with a high number of unique classes, the uncertainty of the ICP classification output may increase because of the low final significant level setting that each class needs to satisfy. 

==> Sections/Section_results_with_lamda.tex <==
\section{Experimental Results}
\label{experimental-results}
This sections describes our experimental set up and presents classification results without the use of ICP, with the use of typical ICP power-set approach on the reduced data-sets and with the use of efficient ICP power-set approach on full data-sets. In experimental set up section we discuss the data-sets and the evaluation metrics used for results and the hardward employed for experiments. 


\subsection{Corpora}\label{corpora}

We present experimental results for three data-sets, two consisting of English-language documents and one consisting of Czech-language documents,  the statistics of which are summarised in Table~\ref{tab:corpora_stats}.
The ``word2vec'' model uses WEs trained on Google News\footnote{\url{https://s3.amazonaws.com/dl4j-distribution/GoogleNews-vectors-negative300.bin.gz}} and on the Czech Wikipedia. The Bert classifier uses $BERT_{base}$ as described in Section \ref{bert_embeddings} and  SlavicBERT\footnote{https://huggingface.co/DeepPavlov/bert-base-bg-cs-pl-ru-cased} \citep{arkhipov2019} which was initializated from multilingual $BERT_{Base}$ and later trained  on Russian News and four Wikipedia versions: Bulgarian, Czech, Polish, and Russian. For all models we use binary cross-entropy~\citep{de2005tutorial} as a loss function, and the Adam~\citep{kingma2014} optimizer. For all experiments, we employ early stopping with patience of 3 epochs based on validation F1-score.

For all data-sets, we have additionally partitioned calibration sets that are necessary for ICP. The calibration documents are selected randomly from the training part with respect to label distributions. The size of calibration data-sets is 999 in all cases apart from the AAPD where it is 4999 because of the huge number of documents it contains. The data-sets CTDC20, Reuters20 and AAPD20 are reduced versions of the full ones, generated by selecting the 20 most frequent classes in all cases. 

\subsubsection{Czech Text Document Corpus v 2.0 (CTDC)}
This corpus\footnote{http://ctdc.kiv.zcu.cz/} consists of real Czech newspaper articles provided by the Czech News Agency~(\v{C}TK)\footnote{https://www.ctk.eu/}. The main part (for training and testing) is composed of 11,955 documents, while the development set contains 2,735 additional articles. The testing protocol assumes a five-fold cross-validation on the main part for training and testing with the use of the development documents as a validation set. The documents belong to different categories such as weather, politics, sport, culture etc. and each document is associated with one or more categories. The corpus was annotated by professional journalists from the Czech News Agency and contains 60 different categories. All documents are automatically morphologically annotated using the UDPipe tool.
%The total number of word tokens is 3,505,965 which represents 150,899 unique words.
%The total category number is 60. %out of which 37 most frequent ones are used for classification.
%The reason of this reduction is to keep only the classes with the sufficient number of occurrences to train the models.

\subsubsection{Reuters 21578}
The Reuters 215782 corpus\footnote{\url{http://www.daviddlewis.com/resources/testcollections/reuters21578/}} is comprised of documents collected from the Reuters news-wire in 1987.
The documents were manually annotated and the initial version of the data-set was further cleaned up in 1996 resulting in the current form. The training-set contains 7,769 documents,  while 3,019 documents are reserved for testing. For our experiments, to be consistent with the other corpora, we have prepared a validation-set containing 1,000 documents taken from the training-set. The documents were selected randomly, but with respect to the training-set's label distributions.
% The numbers of documents are shown in Table~\ref{tab:reuters_stats}.

\subsubsection{Arxiv Academic Paper Dataset (AAPD)}
AAPD\footnote{\url{https://github.com/lancopku/SGM}}~\cite{yang2018sgm} is a relatively new large data-set for multi-label text classification.
%\url{https://github.com/lancopku/SGM}
It is composed of abstracts and corresponding subjects of 55,840 papers in the computer science area collected from the arXiv\footnote{\url{https://arxiv.org/}} website.
There are 54 subjects in total and one research paper usually has multiple subjects.
%The goal is to predict corresponding subjects of an research paper according to the abstract.
This corpus is divided into training, validation and test sets, as described in Table~\ref{tab:corpora_stats}.

\begin{table}
\centering
\footnotesize{
  \caption{Corpora statistics; \textit{Docs} indicates the total number of documents in the corpus, \textit{Test} and \textit{Validation} are sizes of test and validation parts respectively, if available;}
  \label{tab:corpora_stats}
  \begin{tabular}{c|cccccc}
    \hline
    \textbf{Part} & \textbf{Docs} & \textbf{Test} & \textbf{Validation} & \textbf{Labels} & \textbf{avg. labels} & \textbf{avg. words} \\
    \hline
    \hline
    \textbf{CTDC} & 14,690 & - & 2,735 & 60 & 2.64 & 275 \\
    \textbf{CTDC20} & 13,702 & - & 2,397 & 20 & 1.96 & 269 \\
    \hline
    \textbf{Reuters} & 10,788 & 3,019 & - & 90 & 1.24 & 165 \\
    \textbf{Reuters20} & 9,855 & 2,738 & - & 20 & 1.16 & 163 \\
    \hline
    \textbf{AAPD} & 55,840 & 1,000 & 1,000 & 54 & 2.41 & 164 \\
    \textbf{AAPD20} & 52,881 & 944 & 942 & 20 & 1.95 & 165 \\
    \hline
\end{tabular}
}
\end{table}

\subsection{Evaluation Metrics}
\label{evaluation_metrics}
We used typical evaluation metrics for applying ICP in multi-label classification which can be grouped into two categories. The first relates to the performance of the forced-prediction mode which enables the comparison of ICP with the underlying model, while the second category concerns prediction-sets and the quality of p-values. 
In all cases, $\vv{y}_i, \vv{z}_i \subseteq \mathcal{P}(\{\Psi_1,\dots,\Psi_d\})$, where $\vv{y}_i = (t_i^1, \dots, t_i^d) $ corresponds to the true label-set and $\vv{z}_i = (z_i^1, \dots, z_i^d)$ to the predicted label-set for test instance $i\in \{1,\dots,m\}$ which derives from thresholding the raw prediction of the classification process with $0.5$.

Forced-prediction results are evaluated using six different metrics: 

\begin{itemize}
    \item 
    \emph{Classification accuracy $(CA)$} is computed for the complete set of test instances and averaged over their total number. For each instance, a correct prediction is given if and only if the true multi-label target has been fully matched by the highest p-value prediction, i.e. 

    \begin{equation}
        CA = \frac{1}{m}\sum^{m}_{i=1} I(\vv{y}_i=\vv{z}_i),
    \end{equation}{}

    where $I$ is 1 if the condition is true and 0 otherwise. Accuracy is therefore strict and rewards only \emph{absolutely-correct} predictions and not \emph{partially-correct} predictions.

    \item
    The \emph{$F_1$-measure} corresponds to the harmonic mean of precision and recall and its value is in the range [0, 1]. It can be further split into the micro-averaged and macro-averaged types. $F_{micro}$ is averaged over the complete set of test instances, which means that more frequent labels weight more than infrequent ones. Conversely, $F_{macro}$ is first averaged per label and the results are then averaged over the total number of labels. Consequently, $F_{macro}$ gives equal weights to all labels and it therefore tends to be lower than $F_{micro}$ when poorer performance is observed for the more infrequent ones. The two are defined as:
    
    \begin{equation}
    \label{eq:fmicro}
        F_{micro} = \frac{2\sum^{d}_{j=1}\sum^{m}_{i=1}{t_i^j} {{z_i^j}}}{\sum^{d}_{j=1}\sum^{m}_{i=1}t_i^j +\sum^{d}_{j=1}\sum^{m}_{i=1}{z_i^j}},
    \end{equation}{}
    
    \begin{equation}
    \label{eq:fmacro}
        F_{macro} = \frac{1}{d} \sum^d_{j=1} \frac{2\sum^{m}_{i=1}t_i^j z_i^j}{\sum^{m}_{i=1}t_i^j +\sum^{m}_{i=1}z_i^j},
    \end{equation}{}
  
    \item
    \emph{Hamming Loss (HL)} is evaluated as a loss function and, in contrast to accuracy and $F_1$ measures, the objective is minimisation. It is given by the symmetric difference between actual and predicted labels, averaged over the total number of test instances and it is more suitable than $CA$ for multi-label classification problems as it also rewards \emph{partially-correct} predictions. It is defined as: 
    
    \begin{equation}
    \label{eq:hl}
        HL = \frac{1}{md}\sum^m_{i=1}\sum^d_{j=1} t_i^j \oplus z_i^j,
    \end{equation}{} 
    
    where $\oplus$ is the xor operator.
    
    \item
    
    We also evaluate \emph{average-confidence ($\overline{Conf.}$)}, which is intended as an overall indication of how likely predictions are compared to all other possible classifications (Section \ref{sec:conformal-prediction}) and it is defined as: 
    
    \begin{equation}
    \label{eq:conf-criterion}
        \overline{Conf.} = \frac{1}{m}\sum_{i=1}^m 1 - \max_{\vv{Y}_j \neq {\arg\max p_i(\vv{Y}_j)}} p_i(\vv{Y}_j), 
    \end{equation}{}    
    
    where we compute the average value of all confidence scores (i.e. $1 -$ the second largest p-value $p$, over all considered label-sets $\vv{Y}_j)$ over $m$ number of test instances.
    
    \item
    As discussed in Section \ref{sec:conformal-prediction}, credibility indicates how suitable is the training data-set for each test instance. Here we evaluate an overall model suitability using \emph{average-credibility ($\overline{Cred.}$)}, defined as:
    
    \begin{equation}
    \label{eq:cred-criterion}
        \overline{Cred.} = \frac{1}{m}\sum_{i=1}^m \max_{\vv{Y}_j} p_i(\vv{Y}_j), 
    \end{equation}{}
    
    where the credibility of example $i$ is the largest p-value $p$ out of all considered label-sets $\vv{Y}_j$.
    
    
\end{itemize}

\bigbreak

The quality of the generated p-values and the practical usefulness of the prediction-sets are evaluated using the following criteria, as proposed in \citep{cp-criteria}:

\begin{itemize}
    
    \item The \emph{s-criterion (S)}, i.e. sum criterion, is an efficiency measure given as the average sum of p-values across all test instances and it is independent of significance level $\epsilon$. Small values are preferable. It is defined as:

    \begin{equation}
    \label{eq:s-criterion}
        S = \frac{1}{m}\sum^{m}_{i=1}\sum_{\vv{Y}_j} p_i(\vv{Y}_j)
    \end{equation}{}
    
    \item The \emph{of-criterion (OF)}, i.e. observed-fuzziness criterion, is the same as the \emph{s-criterion}, but excluding the p-value of the true label-set. It therefore evaluates the average prediction-set size for all false predictions. Smaller values are, again, preferable. It is defined as:
    
    \begin{equation}
    \label{eq:of-criterion}
        OF = \frac{1}{m}\sum^{m}_{i=1}\sum_{\vv{Y}_j \neq {\vv{y}_i}} p_i(\vv{Y}_j)
    \end{equation}{}
    
    where we sum all p-values $p$ excluding the p-value of the true label-set.
    
    \item 
    The \emph{n-criterion}, i.e. number criterion, which returns the average size of the resulting predictions-sets:

    \begin{equation}
    \label{eq:n-criterion}
        N = \frac{1}{m}\sum^{m}_{i=1}|\Gamma^\epsilon_i|.
    \end{equation}{}
    
    where $|\Gamma^\epsilon_i|$ is the size of the resulting prediction-set for instance $i$ at a significance level $\epsilon$.

    \item 
    The \emph{n-median-criterion}, i.e. number criterion, which returns the middle value separating the greater and lesser halves of the resulting predictions-sets sizes:

    \begin{equation}
    \label{eq:n-criterion-median}
        N - median  = median(\{ |\Gamma^\epsilon_i| , i = 1,\dots,m \}),
    \end{equation}{}
    
    where $|\Gamma^\epsilon_i|$ as above.

\end{itemize}
\bigbreak


\subsection{Classification Results Without ICP}
\label{sec:results_without_icp}
In this section we report results for the underlying classifiers on all three data-sets. The classifiers are trained on the whole training-set (proper training and calibration sets). We present results on the full data-sets in Table~\ref{tab:results_withput_icp}, as well as on the reduced versions (consisting of only the 20 most frequent labels) in Table~\ref{tab:results_withput_icp_20}.
The results indicate that the non-contextualised embeddings based classifiers perform approximately the same while bert surpasses them both, by a large margin. This is in agreement with results from recent studies that have improved the state-of-the-art TC performances using transformer-based classifiers like in \cite{stateoftheart20} where researchers proposed "MAGNET" as a model for state of the art performance in multi-label text classification.  They report F1-micro score of 0.899 and 0.696 and hamming loss score of 0.0029 and 0.0252 for Reuters and AAPD data-set respectively. Thus, to the best our knowledge, the implementation of bert presented in this study slightly surpass the state of the art performance obtain by other researchers in the same data-sets. 


\input{./tables_and_trees/results_without_icp.tex}
\input{./tables_and_trees/results_without_icp_20.tex}

For all experiments apart from CTDC20, F1-macro is much lower than F1-micro which suggests that the classification models have poorer performance for the less frequent classes. For the bert classifier, the difference between F1-micro and F1-macro is less than that of the non-contextualised classifiers, meaning that bert is more efficient in classifying rarely encountered labels. Hamming loss values, on the reduced data-sets, show a small superiority of bert over non-contextualised classifiers in predicting fewer false positive labels. For all classifiers, best performance (accuracy and F1-micro) is achieved on the data-sets of Reuters and Reuters20 which is significantly better than other data-sets and a relatively good performance in general for a multi-label task. This can be, at least partly, attributed to the average number of labels per instance (Reuters20: $1.16$ and Reuters: $1.24$) making its complexity very close to that of a multi-class problem. \par

For the CNN classifiers, the initialisation of the embedding layer with word2vec embeddings does not seem to add any performance gain in comparison to the random initialisation when the embedding layer and the task-specific layers are trained (fine-tuned for the case of word2vec) simultaneously. On the contrary, the word2vec classifier performs slightly worst than randinit. This is consistent with results from \cite{lenc2017word}, where authors concluded that for longer texts better results are achieved using embeddings initialised randomly and trained jointly with the classification network.\par

Classification results for the reduced data-sets are significantly better compared to the results from the full versions, as expected based on the fact that the reduced data-sets actually correspond to an easier classification problem (fewer number of possible labels and label-combinations). For data-sets AAPD20 and CTDC20 that have the same average number of labels per instance ($1.96$ and $1.95$, respectively) there is a significant difference in accuracy and F1-micro in favour of CTDC20, despite the fact that AAPD20's total number of training instances is almost 5 times greater than CTDC20. A possible explanation for this -- apart from the distribution of labels -- is that in the case of CTDC20 the average number of words per document is much higher (269 over 165), thus providing richer feature inputs to the model.\par 

\subsection{ICP Power-set}

\subsubsection{Forced Prediction Results}
We apply ICP based on the three classifiers to the data-sets of Reuters20, AAPD20 and CTDC20. 
We present forced-prediction results in Table \ref{tab:forced_prediction_results}, estimated from the label-sets with the highest p-value, as described in Section \ref{sec:conformal-prediction}.\par

\input{./tables_and_trees/forced_prediction_results.tex}

Using Table~\ref{tab:results_withput_icp_20}, a direct performance comparison between the underlying classifiers with and without the use of ICP is possible. This shows that the performance of forced-prediction is negligibly different from the non-ICP classification, for all data-sets, and indicates that no substantial classification performance is sacrificed by the use of ICP. \par

In all cases $\overline{Conf.}$ is relatively high considering the huge number of possible label-sets, which is also reflected in the corresponding accuracy values. The very high values of both accuracy and $\overline{Conf.}$ for the Reuters20 data-set are attributed to its lower complexity due to the low cardinality of its label-sets. $\overline{Cred.}$ is sufficiently high, indicating that the classifiers used are suitable for classifying the test instances. Nonconformity metrics $L_4,\lambda = 0$ and $L_4,\lambda = 1$ do not differ in $\overline{Conf.}$ and $\overline{Cred.}$ measurements meaning that the penalty factor added to the last nonconformity measure does not affect the certainty level and the suitability of the model.

% Not sure if the above is sufficient...


\subsubsection{Prediction Sets Results}
\label{prediction_sets_results}
%Start here with a sentence about the prediction set results. Add a subsection for the S and OF criteria and start it properly!
Lower values are preferred for the $S$ and $OF$ criteria as this indicates that the average p-values of $\vv{Y}_j$ among all instances are kept small, leading to narrower prediction-sets (smaller $n$ criterion). The results for  the $S$ and $OF$ criteria are presented in Table \ref{tab:s_and_of_criteria}. In all cases the $S - OF$ difference is around 0.5 as expected, since the average p-values of the true labels are expected to be 0.5. The nonconformity metric $L_4, \lambda = 1$ offers lower $S$ criteria values than $L_4, \lambda = 0$ indicating that the penalty factor added acts in a beneficial way. In addition, for the nonconformity metrics $L_2, L_4, L_8$ with $ \lambda = 0$ the lower $S$ criterion values are obtained from $L_8, \lambda = 0$ indicating that a high p factor for $L_p$ norm adds value in the ICP process.

\subsubsection*{N and N-median Criteria}
\label{n_and_n_median_criteria}
This section presents the results for the n and n-median criteria. Figures \ref{fig:Reuters20_n} and \ref{fig:Reuters20_median}  are for the Reuters20 data-set, Figures \ref{fig:AAPD20_n} and \ref{fig:AAPD20_median} for the AAPD20 data-set and Figures \ref{fig:CTDC20_n} and \ref{fig:CTDC20_median} for the CTDC20 data-set.\par

In almost all cases, the median prediction-set sizes are smaller than or equal to  the n criterion, for significant levels $\leq 0.05$, which points to extreme values of prediction-set sizes for specific test instances and high confidence levels. For all cases examined, nonconformity metric $L_2, \lambda = 0$ mark the worst performance, while the best performance was achieved by either $L_8, \lambda = 0$ or $L_4, \lambda = 1$. In addition nonconformity metric $L_4, \lambda = 1$ obtained slightly better or equal values with $L_4, \lambda = 0$. With the above observations we can conclude that the use of the penalty factor as well as the increase of the p factor in $L_p$ norm leads to tighter prediction sets, also supported from  the observations pointed out for the $S$ and $OF$ criteria. \par

\input{./tables_and_trees/s_and_of_criteria.tex}


On Reuters20,  the best performance is achieved using the nonconformity metric $L_4, \lambda = 1$. For significant level, $\epsilon = 0.01$, classifiers bert, randint and word2vec produced n criterion values of 13, 36 and 20, respectively. For $\epsilon = 0.05$, the corresponding values are 1.22 for bert, 1.85 for randinit and 1.67 for word2vec. The prediction sets are tight enough to be useful in practise for high confidence levels ($\geq 0.95)$, especially when considering the total number of possible combinations, $c = 137979$.\par

On data-sets AAPD20 and CTDC20 the best performances achieved, for almost all cases, were with nonconformity metric $L_8, \lambda = 0$. For $\epsilon = 0.05$ on the AAPD20 data-set, classifiers bert, randinit and word2vec marked n criterion values of 50, 118 and 178, respectively, while the corresponding values for the CTDC20 data-set were 46, 64 and 63. \par

Prediction sets obtained from bert classifier were significantly tighter compared to randinit and word2vec, for significance levels $\leq 0.05\%$. Additionally, prediction sets sizes of randint and word2vec were roughly the same. We can therefore conclude that prediction sets of ``better'' classifiers, in terms of performance, are tighter, as was implied from the ICP framework. 
\par

%\clearpage

% Reuters20 n and n median
\begin{figure}[!ht]
  \caption{Average Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,keepaspectratio]{img/Reuters20_n.png}
  \label{fig:Reuters20_n}
\end{figure}

\begin{figure}[!ht]
  \caption{Median Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/Reuters20_median.png}
  \label{fig:Reuters20_median}
\end{figure}

\clearpage

% AAPD20 n and n median
\begin{figure}[!ht]
  \caption{Average Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/AAPD20_n.png}
  \label{fig:AAPD20_n}
\end{figure}

\begin{figure}[!ht]
  \caption{Median Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/AAPD20_median.png}
  \label{fig:AAPD20_median}
\end{figure}

\clearpage

% CTDC20 n and n median
\begin{figure}[!ht]
  \caption{Average Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/CTDC20_n.png}
  \label{fig:CTDC20_n}
\end{figure}

\begin{figure}[!ht]
  \caption{Median Prediction-Set Size}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/CTDC20_median.png}
  \label{fig:CTDC20_median}
\end{figure}

\clearpage


\subsubsection*{Empirical Error Rate}
We also examine the empirical validity of our conformal predictors, by plotting the test-sets error-rate against  the  significance  level  in  the  range  $[0, 1]$. Results for the data-sets: Reuters20, AAPD20 and CTDC20 are presented in Figures: \ref{fig:Reuters20_errors},  \ref{fig:AAPD20_errors} and \ref{fig:CTDC20_errors}, respectively. It is shown that, as  guaranteed  theoretically, the error-rate is always less than or equal to the significance level (up to statistical fluctuations) and confirms that our data satisfies the exchangeability assumption.\par

Results reveal an interesting observation for nonconformity metric $L_8, \lambda = 0$ for significant levels $\geq 0.7$. There are cases in the CTDC20 and Reuters20 data-sets where the empirical error-rate deviates from the diagonal, but is still valid since it is below it. A possible explanation can be found in the $L_8$ norm itself, which tends to act like $L_{\inf}$ norm, i.e. it only takes into account the label with the larger prediction error neglecting information from other labels and therefore the nonconformity scores $\alpha_i$ of the  calibration instances $x_i$, only reaches up to a certain magnitude.

% Error rates
\begin{figure}[h]
  \caption{Empirical Error Rate}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/Reuters20_errors.png}
  \label{fig:Reuters20_errors}
\end{figure}


\begin{figure}
  \caption{Empirical Error Rate}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/AAPD20_errors.png}
  \label{fig:AAPD20_errors}
\end{figure}

\begin{figure}
  \caption{Empirical Error Rate}
  \centering
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{img/CTDC20_errors.png}
  \label{fig:CTDC20_errors}
\end{figure}


\clearpage
\subsection{Efficient ICP Power-set in Full Data-sets}
\label{sec:efficient-icp-power-set-in-full-data-set}

asdf
\subsubsection{Forced Prediction Results}
\label{sec:efficient-forced-prediction-results}
asdf
\subsubsection{Prediction-set Results}
\label{sec:efficient-prediction-set-results}
Empirical Results
% We probably need to add more here!

% I am not sure if this is a good introductions to the Results section.
% Can't we simply say that we applied the above method to the full Reuters dataset?

% We obtained predictions set for $\epsilon_0 = 0.05$, using the bert, randint and word2vec underlying classifiers (as descripted in Section \ref{text_classification_overview}) for data-sets Reuters20, AAPD20 and CTDC20. These prediction sets contain exactly the same categories as the ones obtained using the power-set approach, with $t$ consideration, as presented in Section \ref{prediction_sets_results}. 

% We also attempt to obtain results for the full data-sets of Reuters, AAPD and CTDC. Because of implementation difficulties like RAM memory limitations and lack of computation time we were only able to present results for the full Reuters (Table \ref{tab:ICP_Reuters}) data-set for the nonconformity metric. % For which nonconformity metric?

We present experimental results for the full Reuters 21578 data-set (Table \ref{tab:ICP_Reuters}), using the approach outlined above. These results demonstrate that, even for data-sets with a large number of labels ($d=90$) and consequently possible label-set combinations ($>>1e+16$), the application of ICP (i) is not prohibitively computationally expensive, (ii) can produce practically useful prediction sets.\par 

We can also observe that the prediction set sizes are much more heavily depended on the performances of the underlying classifiers, compared to what has been the case during our previous experiments in Section \ref{prediction_sets_results}. 

\input{./tables_and_trees/ICP_on_Reuters.tex}

% Results show that even for data-sets with large number of labels, i.e. $d=90$, where the possible number of classification using the typical power set approach, with $t$ consideration is $>>1e+17$ the application of ICP (i)can be done, (ii) can produce useful in practise prediction sets. An interesting observation is that prediction set size gets much more depended on the performance of the underlying classifier as was indicated from the results in Section \ref{prediction_sets_results}. 

